Revisiting the Sliced Wasserstein Kernel for persistence diagrams: a Figalli-Gigli approach

The Sliced Wasserstein Kernel (SWK) for persistence diagrams was introduced in (Carri{\`e}re et al. 2017) as a powerful tool to implicitly embed persistence diagrams in a Hilbert space with reasonable distortion. This kernel is built on the intuition that the Figalli-Gigli distance-that is the partial matching distance routinely used to compare persistence diagrams-resembles the Wasserstein distance used in the optimal transport literature, and that the later could be sliced to define a positive definite kernel on the space of persistence diagrams. This efficient construction nonetheless relies on ad-hoc tweaks on the Wasserstein distance to account for the peculiar geometry of the space of persistence diagrams. In this work, we propose to revisit this idea by directly using the Figalli-Gigli distance instead of the Wasserstein one as the building block of our kernel. On the theoretical side, our sliced Figalli-Gigli kernel (SFGK) shares most of the important properties of the SWK of Carri{\`e}re et al., including distortion results on the induced embedding and its ease of computation, while being more faithful to the natural geometry of persistence diagrams. In particular, it can be directly used to handle infinite persistence diagrams and persistence measures. On the numerical side, we show that the SFGK performs as well as the SWK on benchmark applications.

==> defs.tex <==
%%% Letters and numbers
% symbols =======================
% https://tex.stackexchange.com/questions/564216/newcommand-for-each-letter
\makeatletter
\newcommand\definealphabetloop[3]{%
  \ifx\relax#3\expandafter\@gobble\else\expandafter\@firstofone\fi
  {\expandafter\providecommand\expandafter*\csname#1#3\endcsname{#2{#3}}%
   \definealphabetloop{#1}{#2}}%
}%
\newcommand\definealphabet[2]{%
  \definealphabetloop{#1}{#2}abcdefghijklmnopqrstuvwxyzABCDEFGHIJKLMNOPQRSTUVWXYZ\relax
}%
\definealphabet{b}{\mathbb}%
\definealphabet{c}{\mathcal}%
\definealphabet{f}{\mathfrak}%
\definealphabet{r}{\mathrm}%
\definealphabet{s}{\mathscr}%
\definealphabet{t}{\mathtt}%
\definealphabet{B}{\mathbf}%
\makeatother

%%%%ù

\newcommand{\bmu}{\bm{\mu}}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\ones}{\mathbf{1}}

\renewcommand{\epsilon}{\varepsilon}

%% Important TDA related notations
\newcommand{\groundspace}{\Omega}
\newcommand{\thediag}{\partial \groundspace}
\newcommand{\quotient}[1]{\tilde{#1}}
\newcommand{\SFG}{\mathrm{SFG}}

%%% General maths notations
\newcommand{\dd}{\mathrm{d}}  % Integration
\newcommand{\prob}{\mathbb{P}}  % Proba of something
\newcommand{\perm}{\mathfrak{S}}  % Set of permutations
\newcommand{\diam}{\mathrm{diam}}  % Diam of a set
\newcommand{\supp}{\mathrm{spt}}
\newcommand{\mean}{\mathrm{mean}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\Lip}{\mathrm{Lip}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\vspan}{\mathrm{span}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\Div}{\mathrm{Div}}

\newcommand{\p}[1]{\left(#1\right)}

%%% Mesure and OT related notations
\newcommand{\cvvague}{\xrightarrow{v}}
\newcommand{\cvweak}{\xrightarrow{w}}
\newcommand{\cvu}{\xrightarrow{\|\cdot\|_\infty}}

\newcommand{\Adm}{\mathrm{Adm}}  % Set of admissible transport plans
\newcommand{\Opt}{\mathrm{Opt}}  % Set of optimal transport plans

\newcommand{\KL}{\mathrm{KL}}
\newcommand{\MMD}{\mathrm{MMD}}
\newcommand{\TV}{\mathrm{TV}}

\newcommand{\OT}{\mathrm{OT}}
\newcommand{\FG}{\mathrm{FG}}
\newcommand{\SW}{\mathrm{SW}}
%%% Maths operators
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\minimize}{minimize}

%%% Useful additional shortcuts
\newcommand{\gudhi}{\href{https://gudhi.inria.fr/}{\texttt{Gudhi}}}
\newcommand{\pot}{\href{https://pot.readthedocs.io/en/stable/}{\texttt{POT}~}}
\newcommand{\Cech}{\v Cech}
\newcommand{\PersLay}{\textsc{PersLay}}
\newcommand{\proj}{\mathrm{proj}}

\newcommand{\mspt}{\tilde{\mathrm{spt}}}

%%% Misc
%\newcommand{\todo}[1]{\textbf{\textcolor{red}{#1}}}
\newcommand{\theo}[1]{\todo{Théo : #1}}
